Multiplicities in GGGRs for Classical Type Groups with Connected Centre I

Assume $G$ is a connected reductive algebraic group defined over $\bar{\mathbb{F}_p}$ such that $p$ is good prime for $G$. Furthermore we assume that $Z(G)$ is connected and $G/Z(G)$ is simple of classical type. Let $F$ be a Frobenius endomorphism of $G$ admitting an $\mathbb{F}_q$-rational structure $G^F$. This paper is one of a series whose overall goal is to compute explicitly the multiplicity $< D_0745664 {G^F}(\Gamma_u),\chi>$ where: $\chi$ is an irreducible character of $G^F$, $D_{G^F}(\Gamma_u)$ is the Alvis--Curtis dual of a generalised Gelfand--Graev representation of $G^F$ and $u \in G^F$ is contained in the unipotent support of $\chi$. In this paper we complete the first step towards this goal. Namely we explicitly compute, under some restrictions on $q$, the scalars relating the characteristic functions of character sheaves of $G$ to the almost characters of $G^F$ whenever the support of the character sheaf contains a unipotent element. We achieve this by adapting a method of Lusztig who answered this question when $G$ is a special orthogonal group $\SO_{2n+1}(\mathbb{K})$. Consequently the main result of this paper is due to Lusztig when $G = \SO_{2n+1}(\mathbb{K})$.

==> sections/symbols.tex <==
%!TEX root = ../multiplicites-in-GGGRs.tex
%
\section{Symbols}
Extra Information for determining the above Inequalities. Note that in types $\B_n$ and $\D_n$ we have $\Lambda^i\oplus\Lambda^0 = \Lambda^0\oplus\Lambda^i$ for all $i$, in particular the information below deals with both the cases $a'=0$ and $b'=0$.

\begin{description}
	\item[Type $\B_n$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^1,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+4\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^2,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+2,2t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^3,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,3
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^4,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	1,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^5,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+3\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^6,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^7,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)
	\end{align*}
	%%%%
	From this we obtain that the entries of the symbols $\Lambda^i\oplus\Lambda^0$ arranged as increasing sequences are given as follows
	%%%%
	\begin{align}
	&0 \leqslant 0 \leqslant 2\leqslant 2 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 4t \leqslant 4t+2 \leqslant 4t+4\tag{$\Lambda^0\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 2 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 4t \leqslant 4t+2 \leqslant 4t+6\tag{$\Lambda^1\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 2 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 4t \leqslant 4t+3 \leqslant 4t+5\tag{$\Lambda^2\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 4 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 4t \leqslant 4t+2 \leqslant 4t+4\tag{$\Lambda^3\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2 \leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 4t \leqslant 4t+2 \leqslant 4t+4\tag{$\Lambda^4\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 4t \leqslant 4t+2 \leqslant 4t+5\tag{$\Lambda^5\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 2 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 4t \leqslant 4t+2 \leqslant 4t+5\tag{$\Lambda^6\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 4t \leqslant 4t+2 \leqslant 4t+4\tag{$\Lambda^7\oplus\Lambda^0$}
	\end{align}
	
	\item[Type $\C_n$, $d = 4t+1$, $b'=0$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^1,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^2,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t+1,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^3,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,3
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^4,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	1,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^5,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^6,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^7,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)
	\end{align*}
	%%%%
	From this we obtain that the entries of the symbols $\Lambda^i\oplus\Lambda^0$ arranged as increasing sequences are given as follows
	%%%%
	\begin{align}
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+4\tag{$\Lambda^0\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+6\tag{$\Lambda^1\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+3 \leqslant 8t+5\tag{$\Lambda^2\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 4 \leqslant 5 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+4\tag{$\Lambda^3\oplus\Lambda^0$}\\
	&0 \leqslant 2 \leqslant 2\leqslant 4 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+4\tag{$\Lambda^4\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 4 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+4\tag{$\Lambda^5\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+5\tag{$\Lambda^6\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 4 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+4\tag{$\Lambda^7\oplus\Lambda^0$}
	\end{align}
	
\item[Type $\C_n$, $d = 4t-1$, $b'=0$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^1,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^2,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t+1,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^3,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,3
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^4,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	1,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^5,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^6,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^7,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)
	\end{align*}
	%%%%
	From this we obtain that the entries of the symbols $\Lambda^i\oplus\Lambda^0$ arranged as increasing sequences are given as follows
	%%%%
	\begin{align}
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+1\tag{$\Lambda^0\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+3\tag{$\Lambda^1\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t \leqslant 8t+2\tag{$\Lambda^2\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 3\leqslant 4 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+1\tag{$\Lambda^3\oplus\Lambda^0$}\\
	&1 \leqslant 1 \leqslant 3\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+1\tag{$\Lambda^4\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 3\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+2\tag{$\Lambda^5\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+2\tag{$\Lambda^6\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 3\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+1\tag{$\Lambda^7\oplus\Lambda^0$}
	\end{align}

\item[Type $\C_n$, $d = 4t+1$, $a'=0$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^1) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+4\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^2) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+2,4t+3\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^3) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,3
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^4) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	1,2
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^5) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+3\\
	0,2
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^6) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+3\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^7) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,2
	\end{pmatrix}\right)
	\end{align*}
	%%%%
	From this we obtain that the entries of the symbols $\Lambda^0\oplus\Lambda^i$ arranged as increasing sequences are given as follows
	%%%%
	\begin{align}
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+1 \leqslant 8t+3\tag{$\Lambda^0\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+6\tag{$\Lambda^0\oplus\Lambda^1$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+3 \leqslant 8t+5\tag{$\Lambda^0\oplus\Lambda^2$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 4 \leqslant 5 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+4\tag{$\Lambda^0\oplus\Lambda^3$}\\
	&0 \leqslant 2 \leqslant 2\leqslant 4 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+4\tag{$\Lambda^0\oplus\Lambda^4$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 4 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+5\tag{$\Lambda^0\oplus\Lambda^5$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+5\tag{$\Lambda^0\oplus\Lambda^6$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 4 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t \leqslant 8t+2 \leqslant 8t+4\tag{$\Lambda^0\oplus\Lambda^7$}
	\end{align}
	
\item[Type $\C_n$, $d = 4t-1$, $a'=0$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^1) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^2) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^3) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,3
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^4) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	1,2
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^5) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t+1\\
	0,2
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^6) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^7) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,2
	\end{pmatrix}\right)
	\end{align*}
	%%%%
	From this we obtain that the entries of the symbols $\Lambda^0\oplus\Lambda^i$ arranged as increasing sequences are given as follows
	%%%%
	\begin{align}
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+1\tag{$\Lambda^0\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+3\tag{$\Lambda^0\oplus\Lambda^1$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t \leqslant 8t+2\tag{$\Lambda^0\oplus\Lambda^2$}\\
	&0 \leqslant 1 \leqslant 3\leqslant 4 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+1\tag{$\Lambda^0\oplus\Lambda^3$}\\
	&1 \leqslant 1 \leqslant 3\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+1\tag{$\Lambda^0\oplus\Lambda^4$}\\
	&0 \leqslant 1 \leqslant 3\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+2\tag{$\Lambda^0\oplus\Lambda^5$}\\
	&0 \leqslant 1 \leqslant 2\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+2\tag{$\Lambda^0\oplus\Lambda^6$}\\
	&0 \leqslant 1 \leqslant 3\leqslant 3 \leqslant 5 \leqslant 7 \leqslant 9 \leqslant \cdots \leqslant 8t-3 \leqslant 8t-1 \leqslant 8t+1\tag{$\Lambda^0\oplus\Lambda^7$}
	\end{align}
	
	\item[Type $\D_n$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^1,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^2,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t+1,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^3,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,3
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^4,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	1,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^5,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^6,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^7,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)
	\end{align*}
	%%%%
	From this we obtain that the entries of the symbols $\Lambda^i\oplus\Lambda^0$ arranged as increasing sequences are given as follows
	%%%%
	\begin{align}
	&0 \leqslant 0 \leqslant 2\leqslant 2 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t-2 \leqslant 8t \leqslant 8t+2\tag{$\Lambda^0\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 2 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t-2 \leqslant 8t \leqslant 8t+4\tag{$\Lambda^1\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 2 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t-2 \leqslant 8t+1 \leqslant 8t+3\tag{$\Lambda^2\oplus\Lambda^0$}\\	
	&0 \leqslant 0 \leqslant 2 \leqslant 4 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t-2 \leqslant 8t \leqslant 8t+2\tag{$\Lambda^3\oplus\Lambda^0$}\\
	&0 \leqslant 1 \leqslant 2 \leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t-2 \leqslant 8t \leqslant 8t+2\tag{$\Lambda^4\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t-2 \leqslant 8t \leqslant 8t+3\tag{$\Lambda^5\oplus\Lambda^0$}\\
	&0 \leqslant 0 \leqslant 2 \leqslant 2 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t-2 \leqslant 8t \leqslant 8t+3\tag{$\Lambda^6\oplus\Lambda^0$}\\	
	&0 \leqslant 0 \leqslant 2 \leqslant 3 \leqslant 4 \leqslant 6 \leqslant 8 \leqslant \cdots \leqslant 8t-2 \leqslant 8t \leqslant 8t+2\tag{$\Lambda^7\oplus\Lambda^0$}
	\end{align}
	%%%%
\end{description}

\newpage\subsection{Order of $\mathcal{J}$ and $\mathcal{K}$}
\noindent Extra Information for computing the cardinalities of $\mathcal{J}$ and $\mathcal{K}$.

\begin{description}
	\item[Type $\B_n$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\}  \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\}  \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	%%%%	
	(\Lambda^1,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+4\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+4\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	%%%%
	(\Lambda^2,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+2,2t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+2\} \leqslant \{2t+3\} \\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\}  \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	%%%%
	(\Lambda^3,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,3
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 2\} \leqslant \{3 \leqslant 3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2 \leqslant 3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	%%%%
	(\Lambda^4,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	1,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2 \leqslant 2\} \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1 \leqslant 2\}  \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	%%%%
	(\Lambda^5,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+3\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 2 \leqslant 2\} \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+3\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1 \leqslant 2\}  \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	%%%%
	(\Lambda^6,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+3\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	%%%%
	(\Lambda^7,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,2t,2t+1,2t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 2 \leqslant 2\} \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1 \leqslant 2\}  \leqslant \{3\} \leqslant \cdots \leqslant \{2t\} \leqslant \{2t+1\} \leqslant \{2t+2\}
	\end{align*}
	%%%%
	and from this we see that each pair determines $2t+1$ non-degenerate equivalence classes of $\mathbb{L}$. Hence we get $|\mathcal{J}| = 2^{2t}$.
	
	\item[Type $\C_n$, $d = 4t+1$, $b'=0$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	%%%%
	(\Lambda^1,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+3\}\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	%%%%
	(\Lambda^2,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t+1,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	%%%%
	(\Lambda^3,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,3
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1\} \leqslant \{2\} \leqslant \{3 \leqslant 3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3 \leqslant 4\} \leqslant \{5\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	%%%%
	(\Lambda^4,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	1,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^5,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1\} \leqslant \{2 \leqslant 2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+2\}\\
	&\{0 \leqslant 1 \leqslant 1\} \leqslant \{2 \leqslant 3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	%%%%
	(\Lambda^6,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+2\}\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	%%%%
	(\Lambda^7,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1\} \leqslant \{2 \leqslant 2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1 \leqslant 1\} \leqslant \{2 \leqslant 3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}
	\end{align*}
	%%%%
	and from this we see that each pair determines $4t+1$ non-degenerate equivalence classes of $\mathbb{L}$ and no degenerate equivalence classes. Of those equivalence classes precisely 1 is of even order. Hence we get $|\mathcal{J}| = 2^{4t-1}$ and $|\mathcal{K}| = 2^{2t-1}$.
	
	\item[Type $\C_n$, $d = 4t-1$, $b'=0$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}\\
	%%%%
	(\Lambda^1,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+3\}\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}\\
	%%%%
	(\Lambda^2,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t+1,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}\\
	%%%%
	(\Lambda^3,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,3
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1\} \leqslant \{2 \leqslant 3\} \leqslant \{3\} \leqslant \{4\} \leqslant \{5\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0\}\leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}\\
	%%%%
	(\Lambda^4,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	1,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^5,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1\} \leqslant \{2 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+2\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}\\
	%%%%
	(\Lambda^6,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+2\}\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}\\
	%%%%
	(\Lambda^7,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1\} \leqslant \{2 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}
	\end{align*}
	%%%%
	and from this we see that each pair determines $4t$ non-degenerate equivalence classes of $\mathbb{L}$ and no degenerate equivalence classes of odd cardinality. Hence we get $|X| = 2^{4t-2}$.

\item[Type $\C_n$, $d = 4t+1$, $a'=0$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	(\Lambda^0,\Lambda^1) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+4\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+4\}\\
	%%%%
	(\Lambda^0,\Lambda^2) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+2,4t+3\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+2\} \leqslant \{4t+3\}\\
	%%%%
	(\Lambda^0,\Lambda^3) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,3
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1\} \leqslant \{2 \leqslant 3\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	%%%%
	(\Lambda^0,\Lambda^4) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	1,2
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^5) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+3\\
	0,2
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1\} \leqslant \{2 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+3\}\\
	%%%%
	(\Lambda^0,\Lambda^6) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+3\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+3\}\\
	%%%%
	(\Lambda^0,\Lambda^7) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t,4t+1,4t+2\\
	0,2
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 1 \leqslant 2 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t\} \leqslant \{4t+1\} \leqslant \{4t+2\}
	\end{align*}
	%%%%
	and from this we see that each pair determines $4t+1$ non-degenerate equivalence classes of $\mathbb{L}$ and no degenerate equivalence classes of odd cardinality. Hence we get $|X| = 2^{4t-1}$.
	
\item[Type $\C_n$, $d = 4t-1$, $a'=0$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}\\
	%%%%
	(\Lambda^0,\Lambda^1) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t+2\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t+2\}\\
	%%%%
	(\Lambda^0,\Lambda^2) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	%%%%
	(\Lambda^0,\Lambda^3) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,3
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3 \leqslant 4\} \leqslant \{5\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0 \leqslant 1\} \leqslant \{2\} \leqslant \{3 \leqslant 3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}\\
	%%%%
	(\Lambda^0,\Lambda^4) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	1,2
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^0,\Lambda^5) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t+1\\
	0,2
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1\} \leqslant \{2 \leqslant 3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0 \leqslant 1\} \leqslant \{2 \leqslant 2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t+1\}\\
	%%%%
	(\Lambda^0,\Lambda^6) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0 \leqslant 1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t+1\}\\
	%%%%
	(\Lambda^0,\Lambda^7) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},\begin{pmatrix}
	0,1,2,3,\dots,4t-2,4t-1,4t\\
	0,2
	\end{pmatrix}\right)\\
	&\{0 \leqslant 1 \leqslant 1\} \leqslant \{2 \leqslant 3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0 \leqslant 1\} \leqslant \{2 \leqslant 2\} \leqslant \{3\} \leqslant \cdots \leqslant \{4t-2\} \leqslant \{4t-1\} \leqslant \{4t\}
	\end{align*}
	%%%%
	and from this we see that each pair determines $4t$ non-degenerate equivalence classes of $\mathbb{L}$ and no degenerate equivalence classes of odd cardinality. Hence we get $|X| = 2^{4t-2}$.
	
	\item[Type $\D_n$] The appropriate symbols are given by
	%%%%
	\begin{align*}
	(\Lambda^0,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	%%%%
	(\Lambda^1,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+3\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+3\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	%%%%
	(\Lambda^2,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t+1,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t+1\} \leqslant \{4t+2\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	%%%%
	(\Lambda^3,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,3
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 2\} \leqslant \{3 \leqslant 3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2 \leqslant 3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	%%%%
	(\Lambda^4,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	1,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	%%%%
	(\Lambda^5,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 2 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+2\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	%%%%
	(\Lambda^6,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+2\\
	0,1
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+2\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1\} \leqslant \{2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	%%%%
	(\Lambda^7,\Lambda^0) &= \left(\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,2
	\end{pmatrix},
	\begin{pmatrix}
	0,1,2,3,\dots,4t-1,4t,4t+1\\
	0,1
	\end{pmatrix}\right)\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 2 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}\\
	&\{0 \leqslant 0\} \leqslant \{1 \leqslant 1 \leqslant 2\} \leqslant \{3\} \leqslant \{4\} \leqslant \cdots \leqslant \{4t-1\} \leqslant \{4t\} \leqslant \{4t+1\}
	\end{align*}
	%%%%
	and from this we see that each pair determines $4t$ non-degenerate equivalence classes of $\mathbb{L}$ and at most two degenerate equivalence classes which are of even order. Hence we get $|X| = 2^{4t-2}$.
\end{description}
